Parallel Small Vertex Connectivity in Near-Linear Work and Polylogarithmic Depth

We present a randomized parallel algorithm in the {\sf PRAM} model for $k$-vertex connectivity. Given an undirected simple graph, our algorithm either finds a set of fewer than $k$ vertices whose removal disconnects the graph or reports that no such set exists. The algorithm runs in $O(m \cdot \text{poly}(k, \log n))$ work and $O(\text{poly}(k, \log n))$ depth, which is nearly optimal for any $k = \text{poly}(\log n)$. Prior to our work, algorithms with near-linear work and polylogarithmic depth were known only for $k=3$ [Miller, Ramachandran, STOC'87]; for $k=4$, sequential algorithms achieving near-linear time were known [Forster, Nanongkai, Yang, Saranurak, Yingchareonthawornchai, SODA'20], but no algorithm with near-linear work could achieve even sublinear (on $n$) depth.

==> balanced.tex <==
\section{Parallel s-t Vertex Connectivity and Minimum Balanced Cut}

\yonggang{The general principle is to put a headline and lemma saying what you are going to do in this section in the beginning, instead of jumping into the detail immediately}
In this section, we will prove the following lemma.
\begin{lemma}[Parallel s-t vertex connectivity]\label{lem:parallelstvertexconnectivity}
    There is a randomized \pram{} algorithm given an undirected graph $G=(V,E)$, two vertices $s,t$ and a positive integer $k$, outputs $S\subseteq V-\{s,t\}$ or $\bot$ in $\tO{mk^9}$ work and $\tO{k^9}$ depth\yonggang{Try to fix the polynomial factor on $k$ in the end}. It is guaranteed that
    \begin{itemize}
        \item if the algorithm outputs $S$, then $|S|<k$ and $S$ must be a valid $(s,t)$-separator,
        \item if the algorithm outputs $\bot$, then $s,t$ are $k$-vertex-connected in $G$ w.h.p.
    \end{itemize}
\end{lemma}

\Cref{lem:parallelstvertexconnectivity} immediately gives an algorithm for computing the minimum balanced vertex cut, as shown in the following corollary.

\begin{corollary}[Parallel minimum balanced vertex cut]\label{cor:parallelbalanced}
    There is a randomized \pram{} algorithm given an undirected graph $G=(V,E)$, outputs $S\subseteq V$ or $\bot$ in $\tO{mk^9}$ work and $\tO{k^9}$ depth\yonggang{Try to fix the polynomial factor on $k$ in the end}. It is guaranteed that
    \begin{itemize}
        \item if the algorithm outputs $S$, then $|S|<k$ and $S$ must be a valid vertex cut,
        \item if there exists a vertex cut $(L,S,R)$ of $G$ such that \todo{guarantee for volume of $L,R$ and size of $S$}, then the algorithm output $S$ w.h.p.
    \end{itemize}

\end{corollary}
\begin{proof}
     
    \yonggang{Every lemma, thm, corollary should have a proof}
\end{proof}
\subsection{Parallel s-t Vertex Connectivity}

\yonggang{Write the MWU algorithm for s-t vertex connectivity. I think you need to be careful here to write reasonable lemmas so that you can use in the next section for solving the unbalanced case, because there you also need MWU framework and you might want to avoid re-proving lemmas.}


Given a graph $G = (V, E)$, Let's assume there is a vertex cut $S \subseteq V$ where $(L, S, R)$ is a partition of $V$ and $G[V -S]$ disconnects $L$ and $R$. Without loss of generality we assume $\vol(L) \le \vol(R)$.

For a constant $C$, we call $S$ is a \textbf{balanced cut} if $m \le (k \log n)^{C} \vol(L)$. Otherwise, we call $S$ an \textbf{unbalanced cut}.

\todo{determine value of $C$. I suspect $C = 15$}

For a balanced cut, we rely on the fact that if we sample a pair of vertices $(x, y)$ randomly, it is likely to have $x$ and $y$ on the different side -- one in $L$, and the other in $R$.

Without specific mention, we define \textbf{sampling} of vertices as:
\begin{enumerate}
    \item Sample an edge $e$ with uniform random.
    \item Return one of endpoints of $e$, again with uniform random.
\end{enumerate}

Hence, the sampled pair of vertices $(s, t) \in L \times R$ with probability at least $(k \log n)^{-C}(1 - (k \log n)^{-C})$. Hence if we sample $\tO{(k \log n)^{C}}$ such pairs, we have a desired pair with high probability.

For each pair, we use multiplicative weight framework to obtain a fractional cut. We define a progress \textsc{findfractionalcut}$(s, t)$.

\begin{algorithm}
\caption{\textsc{findfractionalcut}$(s, t)$}
\begin{algorithmic}
    \STATE $w^{0}(v) \gets 1$ for all $v \in V - \{s, t\}$, $w^{0}(s), w^{0}(t) \gets 0$.

    \FOR{$t = 1, \cdots, T$}
        \STATE Find $(1 + \delta)$-shortest path $P^{t}$ from $x$ to $y$ with respect to $w^{t-1}$.
        \STATE $w^{t}(v) \gets (1 + \epsilon)w^{t-1}(v)$ for $v \in P^{i}$. Otherwise, $w^{t}(v) \gets w^{t-1}(v)$.
        \STATE $W^{t} := \sum_{v} w^{t}(v)$.
    \ENDFOR

    \STATE $x(v) := \frac{1}{T}\sum_{i=1}^{T} \frac{w^{t}(v)}{W^{i}}$.
    \RETURN $x$
\end{algorithmic}
\end{algorithm}

Let $P_{x}$ be the shortest $(s, t)$ path according to the vertex weight $x$.
\begin{align}T \cdot x(P_{x}) = \sum_{i=1}^{T} \frac{w^{i}(P_{x})}{W^{i}} \ge \frac{1}{1+\delta}\sum_{i=1}^{T} \frac{w^{i}(P^{i})}{W^{i}} \label{ineq:balanced_upper}
\end{align}

by $(1+\delta)$-approximation of $P^{i}$.

On the other hand, Let $\mathrm{OPT}$ be the maximum value of fractional $(s, t)$-cut. Indeed, $\mathrm{OPT} \ge x(P_{x})$. By no-regret bound, we have a following inequality.

\begin{align}
    \sum_{i=1}^{T} \frac{w^{i}(P^{i})}{W^{i}} \ge T(1 - \epsilon)\mathrm{OPT} - \frac{\log n}{\epsilon} \label{ineq:balanced_lower}
\end{align}

Combining \ref{ineq:balanced_upper} and \ref{ineq:balanced_lower}, one can obtain
\begin{align}
    \mathrm{OPT} \ge x(P_{x}) \ge \frac{1 - \epsilon}{1 + \delta}\mathrm{OPT} - \frac{\log n}{T\epsilon(1+\delta)}
\end{align}

We will choose $T = 64k^{3} \log n$, and $\epsilon^{-1} = \delta^{-1} = 8k$.

\begin{itemize}
    \item If there is no such fractional $(s, t)$ cut, it means $\mathrm{OPT} \le \frac{1}{k}$. Thus we will have $x(P_{x}) \le \frac{1}{k}$.
    \item Otherwise, we have $\mathrm{OPT} \ge \frac{1}{k-1}$. From the inequality above, $x(P_{x}) \ge \frac{8k-1}{8k+1}\mathrm{OPT} - \frac{1}{k(8k+1)} > \frac{1}{k-0.5}$.
\end{itemize}

Thus, we can submit $x$ as a target fractional cut if $x(P_{x}) \ge \frac{1}{k-0.5}$, otherwise we give up.

In total, the work and depth consumed here is majorized by $T$ different run of approximate SSSP. So single invocation of \textsc{findfractionalcut} will take $\tO{m k^{5}}$ work and $\tO{k^5}$ depth.

==> frac_cut.tex <==
\section{Fractional Vertex Cuts}

\todo{This section mainly hold reduction between actual cut and the fractional cut (will be found with MWU) It can rather be a subsection, or just put into preliminaries.}

\yonggang{You can copy the definition from other vertex connectivity papers because we want to follow the convention of terminology. Maybe just copying is not a good idea, but you can copy partially and mimic their format of writing preliminaries. Something that worth noticing: 'vertex cut' usually refers to a tuple $(L,S,R)$, because when we say '(edge) cut' it means $(L,R)$. Other vertex connectivity paper usually call $S$ as 'separator' or $(s,t)$-separator. However, we might also want to call $S$ a vertex cut with a bit abusement of notation, because that's also the convention. Anyway, it's usually a good idea to use the 'reasonable' terminologies of previous papers unless you have a appropriate reason to challenge them. }
\yonggang{Put basic definitions in the preliminaries without definition box (for example usually vertex cut is basic), and more complicated definitions can be postponed to later sections with a definition box.}

In this section, we will extend the notion of vertex cuts to fractional vertex cuts, and demonstrate the reduction of a fractional vertex cut to a vertex cut of equivalent size. In the rest of the paper, all algorithms would output a fractional cut.

\begin{definition}[Fractional Vertex Cut]
    Given a graph $G = (V, E)$ and its two nonempty disjoint vertex subsets $A, B\subseteq V$ with $A, B \neq \emptyset$, $L \cap R = \emptyset$, a \emph{$(A, B)$-fractional separator (or a fractional vertex cut)} is a length function $C: V\to \mathbb{R}_{\ge 0}$ such that, (1) $C(v) =0$ for $v \in A \cup B$ and (2) in the graph $G$ with vertex length $C$, the distance from $A$ to $B$ is at least $1$.
    We use $\sum_{v\in V}C(v)$ to denote the \emph{size} of the fractional vertex cut $C$.
\end{definition}

A \emph{fractional vertex cut} is a triple $(A, C, B)$ such that $C$ is a $(A, B)$ fractional vertex cut. $C$ is a \emph{fractional separator (or a fractional vertex cut)} if there are two disjoint vertex sets $A, B$ such that $C$ is an $(A, B)$-fractional vertex cut.

We prove that fractional vertex cuts naturally extend the vertex cuts.
\begin{lemma}
    Given a graph $G = (V, E)$ with a positive integer $k > 1$ and nonempty disjoint vertex sets $A, B\subseteq V$, there is an $(A, B)$-vertex cut with size $\le k$ if and only if there is a fractional vertex cut with size $\le k + 0.5$. \label{lem:fractional_to_integral}
\end{lemma}

\begin{proof}
    Suppose $S$ is a $(A, B)$-separator of size at most $k$. One can define length function $C$ such that $C(v) = [v \in S]$. It is clear that $C$ is a fractional $(A, B)$ separator of size $\abs{S} < k + 0.5$.

    Suppose $C$ is a fractional $(A, B)$-separator of size at most $k + 0.5$. Given a uniform random number $\theta \in [0, 1]$, define $L_{\theta} := \{ v \mid \dist_{C}(A, v) < \theta\}, R_{\theta} := \{v \mid \dist_{C}(A, v) > \theta + C(v)\}$ and $S_{\theta} = V - (L_{\theta} \cup R_{\theta})$. Since $C$ is an $(A, B)$-separator, $A \subseteq L_{\theta}, B \subseteq R_{\theta}$ for all $\theta \in (0, 1)$. Also, $E[L_{\theta}, R_{\theta}] = \emptyset$. Otherwise, there is an edge $(l, r) \in E[L_{\theta}, R_{\theta}]$. If $P_{l}$ is a shortest $(A, l)$-path, $P_{l} \cup \{r\}$ is an $(A, r)$ path of length $C(P_{l}) + C(r) = \dist_{C}(A, l) + C(r) < \theta + C(r) < \dist_{\ell}(A, r)$, which contradicts to the definition of $R_{\theta}$. Therefore, $S_{\theta}$ is an $(A, B)$-separator.

    Now we estimate the size of $S_{\theta}$. $v \in S_{\theta}$ if and only if $\theta \in [\dist_{C}(A, v) - C(v), \dist_{C}(A, v)]$, thus $\Pr[v \in S] \le C(v)$. $\bbE_{\theta}[\abs{S_{\theta}}] \le \sum_{v \in V} C(v) \le k + 0.5$. Thus, there exists a $\phi \in (0, 1)$ such that $\abs{S_{\phi}} \le k$.
\end{proof}

\begin{corollary}
    Given a graph $G = (V, E)$ with fractional $(A, B)$-separator $C$ of size $\le k + 0.5$, there is a sequential algorithm to output a $(A, B)$-separator of size $\le k$ running in $\tO{m}$ running time.
\end{corollary}

\begin{proof}
    Using Dijkstra's algorithm, one can compute $\dist_{C}(A, v)$ in $\tO{m}$ time. Since $\Pr[S_{\theta} \le k] = 1 - \Pr[S_{\theta} \ge k + 1] = \Omega(k^{-1})$, $\tO{k}$ independent evaluation of $S_{\theta}$ will give a desired sets with high probability within $\tO{nk}$ time. More simply, one can just find $\theta$ such that there are at most $k$ intervals among $[\dist_{C}(A, v) - C(v), \dist_{C}(A, v)]$ contain $\theta$ in $\tO{n}$ time without randomness.
\end{proof}

So given a fractional cut $w$, we can convert this into an actual vertex cut if we can evaluate a single-source shortest path (SSSP) problem. However, there are no known efficient \pram{} algorithm to solve exact SSSP problem. Instead, we will employ an efficient approximate variant of \cite{li2020faster}.



\begin{corollary} \label{cor:vsssp}
    Given a graph $G = (V, E)$ with non-negative vertex weights, there is an algorithm to compute $(1 + \delta)$-approximate SSSP with $\tilde{O}(m/\delta^{2})$ work and $\tilde{O}(1/\delta^{2})$ depth w.h.p.
\end{corollary}

\begin{proof}
    We will compute the shortest path according to the edge weight $\widetilde{w}$ according to \Cref{lem:esptovsp}. Computing $\widetilde{w}$ requires linear work and constant depth, so the overall work and depth is majorized by SSSP, as stated in \Cref{thm:sssp}.
\end{proof}

\begin{lemma} \label{lem:frac2cut}
    Given a fractional vertex cut $(L, w, R)$ with value $\ge 1/(k-0.9)$, there is a randomized \pram{} algorithm to compute a vertex separator with size $<k$ in $\tO{mk^3}$ work and $\tO{k^3}$ depth w.h.p.
\end{lemma}

\begin{proof}
    Let's take the smallest integer $k^{\ast} \le k$ such that the value is greater than equal to $1/(k^{\ast} - 0.9)$. Similarly, we 
    \todo{Complete proof}
\end{proof}

\begin{theorem}
    Given a graph $G = (V, E)$ and a positive integer $k$, there is a randomized \pram{} algorithm with $\tO{mk^9}$ work in expectation and $\tO{k^9}$ depth with high probability, to find $L, R \subseteq V$, and a fractional $(L, R)$ vertex cut $w$ with value $\ge \frac{1}{k - 0.9}$, otherwise state that $G$ is $k$-connected.
\end{theorem}

Combined with the \Cref{lem:frac2cut}, we get the main theorem.


\begin{theorem}\label{thm:main-detail}
    There is a randomized \pram{} algorithm 
    given an undirected graph $G = (V, E)$ and a positive integer $k$, outputs $S\subseteq V$ or $\bot$ in $\tO{mk^{12}}$ work and $\tO{k^{12}}$ depth
    \begin{itemize}
        \item if the algorithm outputs $S$, then $S$ must be a minimum vertex cut of $G$,
        \item if the algorithm outputs $\bot$, then $G$ is $k$-connected w.h.p.\yonggang{Remember to define w.h.p. the first time it appears (define it in the footnote)}
    \end{itemize}
    
\end{theorem}

\todo{add MWU}
